Lieb's concavity theorem, matrix geometric means, and semidefinite optimization

A famous result of Lieb establishes that the map $(A,B) \mapsto \text{tr}\left[K^* A^{1-t} K B^t\right]$ is jointly concave in the pair $(A,B)$ of positive definite matrices, where $K$ is a fixed matrix and $t \in [0,1]$. In this paper we show that Lieb's function admits an explicit semidefinite programming formulation for any rational $t \in [0,1]$. Our construction makes use of a semidefinite formulation of weighted matrix geometric means. We provide an implementation of our constructions in Matlab.

==> research-macros.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{geometry}
%\usepackage{subfigure}

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\J}{\mathcal{J}}

\newcommand{\symdiff}{\Delta}
\newcommand{\prox}{\text{prox}}
\newcommand{\ind}{\perp\!\!\!\perp}
\newcommand{\psd}{\succeq}
\newcommand{\pd}{\succ}
\newcommand{\nsd}{\preceq}
\newcommand{\nd}{\prec}
\newcommand{\tr}{\textup{tr}}
\newcommand{\Pf}{\textup{Pf}}
\newcommand{\Spin}{\textup{Spin}}
\newcommand{\Pin}{\textup{Pin}}
\newcommand{\Cl}{\textup{Cl}}
\newcommand{\rank}{\text{rank}}
\newcommand{\psdcone}[1]{\mathcal{S}_{+}^{#1}}
\newcommand{\sign}{\text{sign}}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\colsp}{\mathcal{R}}
\newcommand{\nullsp}{\mathcal{N}}
\newcommand{\elliptope}{\mathcal{E}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\face}{\mathcal{F}}
\DeclareMathOperator*{\diag}{\text{diag}}
\newcommand{\blkdiag}{\text{blkdiag}}
\newcommand{\subspace}[1]{\mathcal{#1}}
\newcommand{\Sym}{\mathcal{S}}
\newcommand{\Amap}{\mathcal{A}}
\newcommand{\Bmap}{\mathcal{B}}
\newcommand{\shrink}{\text{Sh}}
\newcommand{\proj}{\text{Pr}}
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\newcommand{\spectral}{\text{sp}}
\newcommand{\orthant}[2]{\mathbb{R}^{#1,(#2)}}

\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}
\newtheorem{example}{Example}

